Towards Repairing Neural Networks Correctly

Neural networks are increasingly applied to support decision making in safety-critical applications (like autonomous cars, unmanned aerial vehicles and face recognition based authentication). While many impressive static verification techniques have been proposed to tackle the correctness problem of neural networks, it is possible that static verification may never be sufficiently scalable to handle real-world neural networks. In this work, we propose a runtime verification method to ensure the correctness of neural networks. Given a neural network and a desirable safety property, we adopt state-of-the-art static verification techniques to identify strategically locations to introduce additional gates which "correct" neural network behaviors at runtime. Experiment results show that our approach effectively generates neural networks which are guaranteed to satisfy the properties, whilst being consistent with the original neural network most of the time.

==> 4_exp_old.tex <==
\section{Evaluation}
\label{sec:exp}
We have implemented our approach as a self-contained toolkit called
\textsc{nRepair} with about 2500 source lines of code based on PyTorch,
ONNX\footnote{https://onnx.ai/} and the state-of-the-art analyzer
ERAN\footnote{https://github.com/eth-sri/eran}. The \textsc{nRepair} toolkit as
well as all the data used in our experiments is available
online~\footnote{omitted for anonymity}.  In the following, we evaluate our approach to answer four
research questions (RQs). 
% \noindent \emph{Experimental subjects} 
\subsection{Experimental Setup}
%The following applies to total 40 feed-forward networks with RELU activation functions only.  Other network can be handled
%similarly except using a different way of partitioning the input of a neuron.
Our experiment subjects include 42 feed-forward networks for two kinds of two tasks, i.e., aircraft collision avoidance and image
classification.  The details are shown as follows.
\begin{itemize}
\item \emph{ACAS Xu}. ACAS Xu~\cite{acasxu} is an aircraft collision avoidance system developed for unmanned aircraft. This system
issues appropriate navigation actions to avoid collision with an intruder aircraft based on dynamic programming, which results in
a large numeric lookup table. To compress the lookup table without loss of performance, neural networks are adopted to mimic the
behaviors of the lookup table~\cite{julian2016policy}. Recently, an array of 45 DNNs was developed to reduce the lookup
time~\cite{reluplex}, which are our experiment subjects in this part of the experiment. Each of the fully connected networks has 6
hidden layers and each layer is equipped with 50 ReLU nodes. The inputs of these DNNs consists of five variables describing the
speed and relative position of both the intruder and ownership, and the outputs are the scores of five advisories. These models are subject to a set of 10 safety-critical properties~\cite{reluplex}, which we
adopt to test our approach. 

\item \emph{MNIST}. MNIST~\cite{mnist} is a dataset for image classification, which consists of 70k handwritten digits. Each digit
is represented by a $28\times28$ pixel greyscale image and the range of digits is from 0 to 9. We train three forward neural
networks over this dataset (size of training/test set is 60000/10000) and then evaluate our approach on these models. We refer the
three neural networks as FNNSmall (3 hidden layers), FNNMed (5 hidden layers) and FNNBig (7 hidden layers) respectively, and the
hidden layer size is 100 for all of the three models.  

\item \emph{CIFAR10}. CIFAR10~\cite{cifar10} is another widely used dataset. It contains 60000 32x32 colour images in 10
categories. The dataset is well split, i.e., 50000 training images and 10000 test images. We train three different forward neural
networks over this dataset, and the architectures of the tree networks are same with the architectures of MNIST models described
above. Table~\ref{tab:img-models} shows the details of the image classification models used in our experiments. 

\end{itemize}

\begin{table}[t]
\caption{Neural networks of image classification}
\label{tab:img-models}
{\small \centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Dataset&Model & \begin{tabular}[c]{@{}c@{}}Architecture \\ (layers$\times$ units)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Training \\ Accu.\end{tabular}& \begin{tabular}[c]{@{}c@{}}Test\\ Accu.\end{tabular}\\ \hline
 \multirow{3}{*}{MNIST}                           &FNNSmall &         $3\times100$          &0.9743         &0.9668            \\ 
                             				       &FNNMed   &          $5\times100$          &0.9803         &0.9662         \\ 
                            				       &FNNBig   &           $7\times100$          &0.9671         & 0.9386     \\ \hline
 \multirow{3}{*}{CIFAR10}             &FNNSmall &         $3\times100$          &0.6474         &0.5222           \\ 
                             			        &FNNMed   &          $5\times100$          &0.5689        &0.4966         \\ 
                                                             &FNNBig   &           $7\times100$          &0.6327         &0.4095
                                                             \\ \hline                            
     
\end{tabular}}
\end{table}

\begin{comment}
\begin{table}[t]
\caption{Verification of the ACAS Xu networks}
\label{tab:acasp}
\begin{tabular}{|c|c|c|c|}
\hline
property & Test models  & \#UNSAT \\ \hline
$p_1$ & All 45 models  &  0  \\ \hline
$p_2$ & $N_{x,y}$ for all $x\geq2$ and for all y  &  34  \\ \hline
$p_3$ & All models except $N_{1,7}, N_{1,8}$, and $N_{1,9}$  & 0\\ \hline
$p_4$ & All models except $N_{1,7}, N_{1,8}$, and $N_{1,9}$   & 0 \\  \hline
$p_5$ & $N_{1,1}$  &  0  \\ \hline
$p_6$ & $N_{1,1}$  &  0  \\ \hline
$p_7$ & $N_{1,9}$  & 1  \\ \hline
$p_8$ & $N_{2,9}$  & 1  \\  \hline
$p_9$ & $N_{3,3}$  & 0 \\ \hline 
$p_{10}$ & $N_{4,5}$  & 0  \\ \hline		     				     				     				     
\end{tabular}
\end{table}
\end{comment}

For the ACAS Xu models, among the 45 models and 10 properties, 34 models fail property 2 and 1 model fails property 7 and 1 model
fails property 8, which constitutes a total of 36 repairing tasks. 
%The following evaluation under the ACAS Xu setting is hence conducted on these models and properties. 
For the MNIST and CIFAR10 models, we randomly select multiple images and verify
whether they satisfy local robustness in the $L_\infty$-norm~\cite{cw}, i.e.,
given an image $x$ with label $c$, the $L_\infty$-norm robustness is satisfied
if the model outputs label $c$ for any input in $[x-\tau, x+\tau]$. $\tau$ used
in our experiments is 0.03 for MNIST and 0.0012 for CIFAR10 (i.e.,  maximum
values in DeepPoly). We manage to identify 100 images which violate the property
for both datasets and all models except FNNBig for MNIST, for which a total of
51 images are identified. Note that for the verification of local robustness,
each image together its label is regarded as an independent property, as a
result, we total have 551 repair tasks.

In the following, we report all experiment results. All experiment results are obtained on a workstation with 1 i9-9900 processor and 64GB system memory. The threshold $\alpha$ is set to 5\% of
the number of neurons in the original model, i.e., for all ACAS Xu models, no more than 15 neurons can be modified and for both
MNIST and CIFAR10, the number is 15, 25 and 35 for FNNSmall, FNNMed and FNNBig respectively. The threshold $\beta$ is set to 50
for all experiments, i.e., a neuron can be modified at most 50 times. The values of these two parameters are identified empirically. %\dgl{shall we discuss the two paprameters?}\\
%a maximum of 5\% of the neurons .

%\emph{Repair cases of MNIST and CIFAR10}. The verification on the models from the two dataset is straightforward, i.e., given
%robustness constant $\tau$ and an image $x$ with label $l$, DeepPoly directly performs robustness verification in the input space
%$[x-\tau, x+\tau]$. The $\tau$ used in our experiments is 0.03 for MNIST and 0.0012 for CIFAR10. The two values are the maximum
%values adopted in DeepPoly.  We search the images as the repair cases which satisfy both conditions:  1) violating the
%$L_\infty$-norm robustness property. 2) counterexamples can be found when the violation occurs. We plan to randomly select 100
%desired images from the whole test set for each model, but for the FNNBig only 51 desired images are found due to the size of
%model and the bigger $\tau$ we used.  The third column of Table~\ref{tab:rq1-imgs} summarizes the number of repair cases for
%MNIST. \\


\begin{comment}
\begin{itemize}
\item Is our approach effective at making fault models satisfy a given property?
\item How does the active value $\epsilon$ influence the effectiveness of our approach?
\item What is the time overhead of our approach?
\end{itemize}
RQ1 aims to evaluate the effectiveness of our approach in two different scenarios. After that, RQ2 explores the influence of the
important hyperparameter $\epsilon$, and provide a suggestion about how to choose this parameter in practice. Lastly, we evaluate
the time efficiency of our approach in RQ3. All experiments are carried out on a workstation with 1 Intel Xeon 3.50GHz CPU, 64GB
system memory. 
\end{comment}


\subsection{Research Questions}
In this section, we aim to answer the following research questions by multiple experiments.\\

\noindent \emph{RQ1: Is \textsc{nRepair} effective at repairing neural networks?} To answer this question, we apply
\textsc{nRepair} to the 36 models of ACAS Xu, 3 models of MNIST and 3 models of CIFAR10. The step size $\eta$ used in this research
question is 0.35 for the ACAS Xu models and 0.05 for both MNIST and CIFAR10 models. $\eta$ is the key hyperparameter in our approach
and we explain how to set the value of $\eta$ later. 

The results on repairing the ACAS Xu models are summarized in Table~\ref{tab:rq1-acasxu}, where the third
column shows the number of partitions that need to be repaired. Note that the number of partitions ranges from 2 to 22.
%For the property 2, we generate a counterexample for each repair case for the further repairing. Since the generation of counter examples is time-consuming, for property 7 and property 8, insteadof searching counterexample for all repair cases, we randomly select 11, the average number of repair cases for each model of property 2, repair cases for each of the two properties.
%identify a set of repair cases $R$.  A repair case $r\in R$ can be denoted as a triple: $(\phi, \omega, N)$, where $\phi$ is an
%input region, $\omega$ is an output constraint and $N$ is a target model which violates $\omega$ when given $\phi$. Our goal is
%to modify $N$ such that given $\phi$, the output of $N$ could satisfy the constraint $\omega$.  The DeepPoly adopts different
%verification strategies when verifying models from different tasks. Hence, we use different strategies to identify repair cases
%under different tasks accordingly. \emph{Repair cases of ACASXU}. When verifying the models from ACAS Xu, the DeepPoly firstly
%splits the input regions of the given property into several subregions under the guidance of gradient and then verifies each
%subregion. In this case, a property is satisfied only when all the input subregions are verified successfully, and not satisfied
%when some subregions are failed. Hence in the setting of  ACAS Xu, we identify the repair cases according to the subregions.
%While in the case of MNIST, DeepPoly directly verifies the whole input region without any preprocessing and thus we identify the
%repair cases at the original input region, i.e., the input images. We refer the readers to the implementation of
%DeepPoly\footnote{https://github.com/eth-sri/eran} for more details about the verification. In the following paragraphs, we
%describe our evaluation of ACAS Xu and MINST separately.  
%\gl{We will discuss how to select $\gamma$ later}.
For each partition, we generate a counterexample (by collecting the constraints that a counterexample must satisfy, i.e., the partitioned input constraint as well as the negation of the property, and solving the constraint using mixed integer linear programming solver
Gurobi~\cite{gurobi}), and then solve the optimization problem as described in
Section~\ref{sec:app}. We then report the percentage of partitions which are
successfully repaired in the fourth column, and the number of neurons which are
modified on average to repair each partition. We observe that \textsc{nRepair}
successfully repairs 92.95\% of the partitions, which means that for almost all
of the regions, the neural network is made such that it is guaranteed to satisfy
the property. We remark that for the few regions where we fail to repair, it is
always possible to raise an alarm when an input in that region is received at
runtime. Furthermore, the number of modified neurons are kept relatively small,
i.e., 2.03 on average, or equivalently 0.68\% on average. This suggests that
only minor modifications are required to repair the neural networks. 

The results on repairing the MNIST and CIFAR10 models are summarized in Table~\ref{tab:rq1-imgs}. Note that due to the many repair tasks (i.e., 551 in total), we only show the average success rate and time. Note that these models are
bigger and more complex than those of ACAS Xu. As a result, the number of partitions to be repaired are larger (i.e., 11 partitions on average for each repair task) and overall these,
models are expected to be harder to repair. Our approach achieves 95.52\% success rate on the two datasets on average.
Concretely, it can be observed that the success rate of FNNSmall and FNNMel is nearly 100\% , and for FNNBig the success rate drops but still remains at a relatively high level, i.e, 94.11\% for MNIST and 84\% for CIFAR10. This suggests that our approach has the good scalability, 
in terms of the success rate, and thus has the potential to be applied in practice.
 
% The reason is that because \textsc{nRepair} relies on DeepPoly's verification results to repair the models, it
% fails to repair if DeepPoly fails to provide meaningful verification results, which is the case for bigger models. 
In addition, we observe that the number of modified neurons for those models which we successfully repair is larger than those
for the ACAS XU models, i.e., on average 4.22 and 4.93 neurons are modified. This is reasonable because for a simple model like ACAS XU, a few
neurons can dominate a certain result, whereas for a more complex model like MNIST and CIFAR10, the classification results are typically the joint results of multiple (if not many) neurons.
We thus have the following answer to RQ1.
\begin{framed}
\noindent  \emph{Answer to RQ1: \textsc{nRepair} repairs neural network models with a high success rate and modifies a small number of neurons.}
\end{framed}

\begin{table}[t]
  \centering
  \footnotesize
  \caption{Results of repairing on ACAS Xu models}
\label{tab:rq1-acasxu}%

    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
 Property & Model & \begin{tabular}[c]{@{}c@{}}\#partitions \end{tabular} & \begin{tabular}[c]{@{}c@{}}Success\\
 rate(\%)\end{tabular}  & Avg.m & Avg.f(\%)  \\
    \hline
    \multirow{34}[68]{*}{$p_2$} & $N_{2,1}$ & 11    & 100    & 1.63      &  93.98        \\
                                & $N_{2,2}$ & 20    & 100    & 2.05      &  92.47       \\  
                                & $N_{2,3}$ & 20    & 100    & 1.85  &  96.82    \\
                                & $N_{2,4}$ & 10    & 100    & 1.8  &  95.63   \\
                                & $N_{2,5}$ & 20    & 100    & 1.7  &  97.6       \\
                                & $N_{2,6}$ & 9     & 88.89    & 1.75  &  97.63   \\
                                & $N_{2,7}$ & 9     & 66.67    & 1.83  &  98.01       \\
                                & $N_{2,8}$ & 10    & 100    & 2.4  &  97.42    \\
                                & $N_{2,9}$ & 6     & 100    & 3.83  &  98.34          \\
                                & $N_{3,1}$ & 9     & 100    & 1.44  &  96.01    \\
                                & $N_{3,2}$ & 3     & 100    & 1.67  &  98.38    \\
                                & $N_{3,4}$ & 6     & 100    & 2    &  98.32     \\
                                & $N_{3,5}$ & 7     & 100    & 2  &  97.3     \\
                                & $N_{3,6}$ & 9     & 100    & 1.33  &  96.09     \\
                                & $N_{3,7}$ & 8     & 100    & 1.75  &  95.49    \\
                                & $N_{3,8}$ & 10    & 100    & 2.1  &  96.14     \\
                                & $N_{3,9}$ & 20    & 100    & 3.9  &  97.5       \\
                                & $N_{4,1}$ & 5     & 100     & 1.8  &  98.78    \\
                                & $N_{4,3}$ &20     & 70      & 5.86  &  94.07     \\
                                & $N_{4,4}$ & 9     & 55.56   & 1.6  &  98.43     \\
                                & $N_{4,5}$ & 9     &88.89    & 4.36  &  98.2    \\
                                & $N_{4,6}$ & 10    & 90   & 4  &  98.82   \\
                                & $N_{4,7}$ & 9     & 88.89 & 1.11  &  98.73    \\
                                & $N_{4,8}$ & 9      & 100   & 2.88  &   98.95        \\
                                & $N_{4,9}$ & 4      & 100   & 1.67  &   98.76         \\
                                & $N_{5,1}$ & 22   & 100     & 1.32  &   91.43    \\
                                & $N_{5,2}$ & 20    & 100    & 1.3   &  96.81   \\
                                & $N_{5,3}$ & 2     &100     & 1   &  99.87 \\
                                & $N_{5,4}$ & 9    & 44.44     & 2.25    &  98.68 \\
                                & $N_{5,5}$ & 16    & 93.75    & 1.27   &  97.65 \\
                                & $N_{5,6}$ & 16    & 100    & 1.06   &  98.64 \\
                                & $N_{5,7}$ & 10     & 100   & 1.6  &  98.24 \\
                                & $N_{5,8}$ & 9      & 66.67   & 1.17  &  98.45 \\
                                & $N_{5,9}$   & 9    & 100   & 1.33  &  97.55 \\
                                \hline
                                $p_7$    & $N_{1,9}$    &11      &90.9        &1.6     &99.38  \\
                                \hline
                                $p_8$    & $N_{2,9}$    & 11      & 100    & 1     & 99.33 \\
    \hline
    \multicolumn{3}{|c|}{Avg}   & 92.95    & 2.03    & 97.33\\
    \hline
    \end{tabular}%
% \vspace{-0.1cm}
\end{table}%

\begin{table}[t]
  \centering
  \caption{Results of repairing on image classification}
\footnotesize
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    Dataset & Model & \begin{tabular}[c]{@{}c@{}}\#Repair\\ cases\end{tabular} & \begin{tabular}[c]{@{}c@{}}Success\\
    rate(\%)\end{tabular}  & Avg.m & \begin{tabular}[c]{@{}c@{}}Avg.acc \\ Local(\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.accR \\ Global(\%)\end{tabular}\\
    \hline
\multirow{4}{*}{MNIST}      &FNNSmall & 100   &100     &2.19   & 100 & 98.42 \\ \
    		                    &FNNMed   & 100   &100     &2.95   & 100 & 88.18  \\ \
                            &FNNBig   & 51    &94.11   &7.52   & 100 & 56.71  \ \\  \cline{2-7} 
                            & \multicolumn{2}{|c|}{Avg} &98.04 & 4.22  & 100  &81.1 \\
    \hline
\multirow{4}{*}{CIFAR10}  &FNNSmall   & 100    &97      &3.48   & 100   &81.39 \ \\
    				              &FNNMed     & 100    &98      &4.67   & 100   &69.77 \\\
                          &FNNBig     & 100    &84      &6.63   & 100   &62.15 \ \\  \cline{2-7} 
                          &\multicolumn{2}{|c|}{Avg}    &93    &4.93    & 100 &71.10 \\
    
 \hline    
    \end{tabular}%
   \label{tab:rq1-imgs}%
  %  \vspace{-0.2cm}
\end{table}%

%In general, our approach achieves 99.41\% success rate with 97.58\% fidelity achieved for the ACASXU models, and for MNIST and
%CIFAR10, we achieves the 63.5\% success rate with 70.17\%  of performance of the original model retained, and 58.3\% success rate
%with 74.04\%  of performance of the original model retained respectively. The exceptional performance on ACAS Xu indicates that
%our approach is more suitable for the simple yet practicable scenario. For the small models of both MNIST and CIFAR10, our
%approach also achieves high success rate, i.e., 90\% and 79\% respectively. Interestingly, from Table~\ref{tab:rq1-imgs}, we
%observe that as the increasing size of target model, the success rate as well as the ``accR'' decreases, which provide us  the
%insight that the more complex a model is, the more harder the model to repair (low success rate of repair). This is reasonable
%because our approach depends on the performance of the verifier and existing verifiers usually work not well on complex models.
%We thus have the following answer to RQ1:
% 2) complex models are more sensitive to the modification than the relative simple models (low $accR$ of repaired modelss). 

\begin{comment}
\noindent \emph{RQ2: Does \textsc{nRepair} undermine the performance of the model?} The question asks whether the repaired model
carries the same level of performance while satisfying the property, e.g., whether the repaired model has an accuracy close to the
original model. For the ACAS Xu models, because we do not have the training or test dataset (i.e., we cannot measure the accuracy
of the repaired model), we answer this question by measuring % the A nature way to measure this is to compare the accuracy of those repaired models with that of their original model. We use $accR$ to denote the level that the performance of the original model is retained, which is defined as follows:
%\begin{align} accR = \frac{\textit{accuracy of repaired model}}{\textit{accuracy of original model}} \end{align} However, since
%the data set for ACAS Xu is not publicly available, as a substitution, we thus propose a metric, i.e, 
the fidelity of the repaired model with respect to the original model, which is defined as follows.
\begin{align}
Fidelity = \frac{\sum_{x\in T}\mathcal{I}(\hat{N}(x)=N(x))}{|T|}
\end{align}
where $T$ is a test set and $|T|$ is number of samples in $T$; and $\mathcal{I}(y)$ is an indicator function which equals 1 if $y$
holds and 0 otherwise. That is, we synthesize (based on Gaussian sampling) a test set with 10000 samples for each repair cases.
Given the 10000 samples, we filter those which fail the property (since the prediction results on these samples must change in
order to satisfy the property) and then measure the fidelity. The results are shown in the last column of
Table~\ref{tab:rq1-acasxu}. It can be observed that the fidelity remains across all models, i.e., with an average of 97.33\%.
%We remark that we test the fidelity of ACAS Xu by using an ensemble of original models and repaired models. That is,  given an
%input, if it is located in the originally verified partitions of a property, we then use the original model to predict,
%otherwise, we identify which violated partition it is in and then use the corresponding repaired model to perform the
%prediction.''
For MNIST and CIFAR10, we use the test set to measure the accuracy of those repaired models relative to that of their original
model, which is defined as follows.
\begin{align}
accR = \frac{\textit{accuracy of repaired model}}{\textit{accuracy of original model}}
\end{align}
The results are shown in the column ``Avg.accR" of Table~\ref{tab:rq1-imgs}. It can be observed that the accuracy drops
significantly as the size of the model increases. Our hypothesis is that the neurons of these models are highly coupled with each other and thus the behavior of the model is sensitive to the `repairing'. It thus suggests that we need to explore alternative improved ways to repair the model in such cases. We thus have the following answer to RQ2:
% the influence of a minor modification on a neuron of an earlier layer will be magnified layer-after-layer through the network, and thus a deeper network means a greater magnification. However, we remark that the low accR dose not suggest the low effectiveness of repairing. The goal of our repairing on MNIST and CIFAR10 is to make a given model satisfy the local robustness, instead of using a modifed model 
\begin{framed}
\noindent  \emph{Answer to RQ2: \textsc{nRepair} repaired relatively small models maintaining high level of fidelity/accuracy.}
\end{framed}
\end{comment}

\noindent \emph{RQ2: Does \textsc{nRepair}'s repair undermine the overall performance of the model?} The question asks whether the repaired model, while satisfying the property,
carries the same level of performance , i.e., whether the repaired model has an accuracy close to the original model on those inputs whose prediction results by the original model satisfy the property. In other words, the repair should not undermine the performance of the model on those inputs which are not counterexamples to the property. 
For the ACAS Xu models, because the training or test dataset are not available, we cannot measure the accuracy
of the repaired model directly. We thus answer this question by measuring the fidelity of the repaired model with respect to the original model, which is defined as follows.
\begin{align}
Fidelity = \frac{\sum_{x\in T}\mathcal{I}(\hat{N}(x)=N(x))}{|T|}
\end{align}
where $T$ is a test set and $|T|$ is the number of samples in $T$; and
$\mathcal{I}(y)$ is an indicator function which equals 1 if $y$ holds and 0
otherwise. That is, we synthesize (based on Gaussian sampling) a test set with
10000 samples for each repair case. Algorithm~\ref{alg:gauss} shows the details
about how the test set are synthesized. The algorithm takes three parameters:
the original model $N$, the input constraint $\phi$ and output constraint
$\omega$ of a specified property. We first yield a sample $x$ (line 6-7), and
then check if the generated sample satisfies the output constraint $\omega$
(line 8). If yes, we then add it into the test set $X$. Note that we filter
those samples which fail the given property since the prediction on these
samples are supposed to be modified in order to satisfy the property. After
that, we adopt Algorithm~\ref{alg:predict} to perform the prediction with the
repaired models. The results are shown in the last column of
Table~\ref{tab:rq1-acasxu}. It can be observed that the fidelity remains across
all models, i.e., with an average of 97.33\%.

\begin{algorithm}[t]
  \caption{$synthesize\_acasxu(N, \phi, \omega)$}
  \label{alg:gauss}
  Let $(l_1, u_1), (l_2, u_2), \dots,  (l_5, u_5)$ be the lower bound and upper bound of variable $v_1, v_2, \dots, v_5$ defined by input constraint $\phi$\; 
  Let $(\mu_1, \sigma_1), (\mu_2, \sigma_2), \dots,  (\mu_5, \sigma_5)$ be the mean and standard deviation of
  variable $v_1, v_2, \dots, v_5$ respectively\; 
  Let $X=\{\}$ be the set of generated samples\;
  \While{True}{Let $x$ be an empty array with length 5.\; 
    \For{$i=1$ to $5$ }{
      $x[i] \leftarrow Gaussian(l_i, u_i, \mu_i, \sigma_i)$\;
    } 
     \If{$N(x) \vDash \omega$ }{
      $X \leftarrow X \cup \{x\}$\;
    }
    \If{$|X| == 10000$}{
      \Return{X}\;
      }
  }
  \end{algorithm}

For MNIST and CIFAR10, our goal of repairing is to make the original model
satisfy the local robustness property. That is, we repair the given model around
a set of selected images. To evaluate the the repair results on the two image
classification tasks, we report the accuracy of the model with respects to a set
of testing data containing images which are sampled within the norm, i.e., those
which satisfy the input condition. Note that all samples within the norm
should have the same label as the selected image (at the center of the norm).
% test the repaired model}.  Similar to
% the case of ACAS XU, we then measure the accuracy of the repaired model with
% respect to the original model. 
The results are shown in the second last column
``Avg.acc Local" in Table~\ref{tab:rq1-imgs}. We can observe that the result is
always 100\%. This is expected as the repaired model is guaranteed to label the
images within the norm correctly.

%the
%normal way, like what we do on ACAS XU task, is to obtain a set of test samples and then use the repaired models to
%predict when the input is within the corresponding adversarial region. However, in such way, we can always get 100\%
%fidelity since each repaired model is verified within its adversarial region, i.e., the label of each sample in this region is
%proved to be identical.  
Out of curiosity, we conduct an additional experiment as follows. We sample a set of samples throughout the input space and test the accuracy of the repaired model. Note that this is not how the repaired model is meant to be used since the repair is meant to take effect only for those inputs which satisfy the input constraint of the property. Rather, the goal is to see whether a local repair applies globally.  %To compromise, we thus show the the performance of individual repaired model. 
Concretely, we use the test set to measure the accuracy of those repaired models relative to that of their original model, which is defined as follows.
\begin{align}
accR = \frac{\textit{accuracy of repaired model}}{\textit{accuracy of original model}}
\end{align}
The results are shown in the last column ``Avg.accR Global" of Table~\ref{tab:rq1-imgs}. It can be observed that the accuracy is high for small networks and drops
significantly as the size of the model increases. It suggests that a local repair may work globally only if the model is simple. Our interpretation is that the correlation among different neurons are complicated in large neural networks and a minor modification to some neurons may be easily magnified through the network. This suggests that a localized repair, like in our approach, is more likely to be successful in practice. We thus have the following answer to RQ2.
\begin{framed}
\noindent  \emph{Answer to RQ2: \textsc{nRepair} maintains high level of fidelity/accuracy and a local repair generated by \textsc{nRepair} does not apply globally.}
\end{framed}

%We summarise the process of synthesising ACAS Xu test samples in Algorithm~\ref{alg:gauss}. The inputs of
%Algorithm~\ref{alg:gauss} consist of the the original model $N$, the input constraint $\phi$ and output constraint $\omega$ of
%certain property, and the number of samples to generate $max\_size$.  According to the paper~\cite{reluplex}, the ranges of the
%five input variables are: (0, 62000), (-3.141592, 3.141592), (-3.141592, 3.141592), (0,1200) and (0,1200) respectively. The means
%and standard deviations of the five input variables we used are from the implementation of DeepPoly~\cite{DeepPoly}, and we omit
%these values for the sake of saving space.  \\ 

% Table generated by Excel2LaTeX from sheet 'rq1'

%\begin{table}[t] \centering \caption{Results of repairing on image classification} \scriptsize \begin{tabular}{|c|c|c|c|c|c|}
%  \hline Dataset & Model & \begin{tabular}[c]{@{}c@{}}\#partitions\end{tabular} & Avg.$\epsilon$ &
%  \begin{tabular}[c]{@{}c@{}}Success\\ rate(\%)\end{tabular}  & Avg.accR(\%)  \\
%    \hline \multirow{4}{*}{MNIST}      &FNNSmall & 100   & 1.51  & 90      &97.56  \\
%                                   &FNNMed  & 100    & 1.76  & 75     &76.10  \\
%                                   &FNNBig   & 51      & 2.05  & 13       &36.85  \\  \cline{2-6} & \multicolumn{2}{|c|}{Avg} &
%  1.78  &63.5        &70.17   \\
%    \hline \multirow{4}{*}{CIFAR10}  &FNNSmall & 100   &1.07   &79       &91.90 \\
%                 &FNNMed & 100   &1.1     &66      &75.45\\
%                                  &FNNBig & 100    &0.723      &30        &54.77 \\  \cline{2-6} & \multicolumn{2}{|c|}{Avg}
%  &0.96   &58.33        &74.04 \\
% \hline    
%    \end{tabular}% \label{tab:rq1-imgs}% \end{table}%

%We explain this as follows: for both $N_{1,9}$ of property 7 of ACASEU and FNNBig of MNIST, most inputs can not be verified by
%DeepPoly. Concretely, for $N_{1,9}$ with property 7, the input region was divided into 1440 subregions and about 70\% of these
%subregions failed to be verified, and for FNNBig, about 87\% of the whole 10k test sample failed to satisfy the robustness
%property. 
 
\begin{figure}[t]
  \caption{Average time overhead}
  \includegraphics[width=1\columnwidth, height=0.35\textwidth]{figs/rq3-time.pdf}
  \label{fig:rq3}
\end{figure}


\begin{table*}[t]
  \centering
  \caption{Success rate (\%) with different $\eta$}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
    \multirow{2}[4]{*}{Task} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{Model}} & \multicolumn{10}{c|}{$\eta$} \\ \cline{3-12}
                               &               & 0.05  & 0.1   & 0.15  & 0.2   & 0.25  & 0.3   & 0.35  & 0.4   & 0.45  & 0.5 \\ 
    \hline
    \multirow{3}[6]{*}{ACAS Xu}  & $N_{3,8}$(p2)   & 80     & 100   & 90    &  100  & 100   &  90   & 100   & 90    & 100   & 100 \\ \cline{2-12}
                                & $N_{1,9}$(p7)   & 91     & 91   & 91    & 91    & 91    & 91    & 91    & 91    & 91    & 91 \\ \cline{2-12} 
                                & $N_{2,9}$(p8)   & 100    & 91    & 100   & 91    & 91    & 100   & 100   & 100   & 100   & 100 \\ \hline
    \multirow{3}[6]{*}{MNIST}   & FNNSmall &100   & 100   & 100   & 100   & 100   & 100   & 100   & 100   & 100   & 100 \\ \cline{2-12}
                                & FNNMed   & 100    & 99    & 100   & 99    & 98    & 100   & 98    & 96    & 98    & 99 \\ \cline{2-12}          
                                & FNNBig   & 94     & 82    & 75    & 59    & 55    & 55    & 61    & 59    & 67    & 64 \\ \hline
    \multirow{3}[6]{*}{Cifar10} & FNNSmall & 99  & 99    & 99    & 100   & 100   & 100   & 100   & 100   & 100   & 99 \\  \cline{2-12}
                                & FNNMed   & 98    & 97   & 99    & 97    & 97    & 98     & 98     & 98     & 97    & 98 \\  \cline{2-12} 
                                & FNNBig   & 86    & 87   & 84    & 84    & 83    & 83     & 83     & 82     & 82    & 82 \\     \hline
    \end{tabular}%
  \label{tab:sr}%
\end{table*}%

\begin{figure*}[t]
  \caption{Performance of the repaired models with different $\eta$}
  \includegraphics[width=0.33\textwidth]{figs/rq4/acasxu.pdf}
  \includegraphics[width=0.33\textwidth]{figs/rq4/mnist.pdf}
  \includegraphics[width=0.33\textwidth]{figs/rq4/cifar10.pdf}
  \label{fig:quality}
\end{figure*}

\noindent \emph{RQ3: What is the time overhead of our approach?} The most time-consuming step of our approach is the verification
part, which depends on the verification algorithm, the target model and the property. The current implement of \textsc{nRepair}
employs DeepPoly as the verifier since it is the state-of-the-art. \textsc{nRepair} could be easily refactored to take advantage
of improved neural network verifiers which we foresee will be developed in the future. 

In the following, we report the time taken
by \textsc{nRepair} to repair the models (with the same setting as in RQ1).The results are shown in Figure~\ref{fig:rq3}, where
each bar represents the average time (in minutes) of a successful repair and the percentage shown at the top of each bar is the proportion of
the verification time among the total time. For the ACAS Xu task, we show the results on three properties (i.e., property 2, 7 and 8), and for the image
classification task, we show the results on three kinds of models (i.e., FNNSmall, FNNMed and FNNBig). 

We observe that the time overhead varies across different cases. Concretely, the ACAS Xu models take the most time to repair, i.e.,
7.72 minutes on average. One possible reason is that the verified properties are more complex than the local robustness property
for MNIST and CIFAR10. In general, the more complex the property is, the more difficult it is to verify the model, and thus the
more time \textsc{nRepair} takes. This hypothesis, to some extent, can be evidenced by the time spent on repairing property 7.
According to the definition in~\cite{acasxu}, property 7 is more complex than property 2 and 8 since the verification space
(defined by the input constraint) of property 7 is the largest compared with that of property 2 and 8. We can observe that the repair
of property 7 takes the most time, i.e., 19.02 minutes. Furthermore, it can be observed that the verification time takes up 99.98\% of the repair time
for ACAS Xu, 94.9\% for MNIST and 92.98\% for CIFAR10. As expected, the verification time dominates the total execution time.
 
In general, these models are repaired within minutes, which we believe are acceptable as model training typically takes considerable time and our goal to repair a model
offline before the model is deployed. We thus have the following answer to RQ3.
\begin{framed}
\noindent Answer to RQ3: \textsc{nRepair}'s execution time depends on the underlying verifier and \textsc{nRepair} is able to repair benchmark
models within minutes. 
\end{framed}


% Table generated by Excel2LaTeX from sheet 'costs'
\begin{table*}[t]
  \centering
  \caption{Average costs(minutes) with different $\eta$}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
    \multirow{2}[4]{*}{Task} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{Model}} & \multicolumn{10}{c|}{$\eta$} \\
\cline{3-12}          
                                &              & 0.05  & 0.1   & 0.15  & 0.2   & 0.25  & 0.3   & 0.35  & 0.4   & 0.45  & 0.5 \\ \hline

    \multirow{3}[6]{*}{ACAS Xu} & $N_{3,8}$(p2) & 1.65  & 39.71  & 10.33  & 10.40  & 8.95  & 15.77  & 1.55  & 0.87  & 1.47  & 1.41  \\ \cline{2-12}          
                               & $N_{1,9}$(p7) & 22.99  & 20.38  & 16.19  & 21.94  & 18.76  & 15.16  & 19.06  & 14.52  & 12.89  & 17.68  \\\cline{2-12}          
                               & $N_{2,9}$(p8) & 7.82  & 3.43  & 4.02  & 1.89  & 2.01  & 3.49  & 2.81  & 2.21  & 1.97  & 1.85 \\
    \hline
    \multirow{3}[6]{*}{MNIST} & FNNSmall & 0.04  & 0.03  & 0.03  & 0.02  & 0.02  & 0.02  & 0.02  & 0.02  & 0.02  & 0.02  \\ \cline{2-12}          
                              & FNNMed & 0.32  & 0.39  & 0.66  & 0.68  & 0.83  & 0.83  & 0.98  & 0.79  & 0.56  & 0.59 \\ \cline{2-12}          
                              & FNNBig & 4.43  & 1.79  & 2.81  & 1.45  & 0.52  & 1.26  & 1.22  & 2.09  & 0.78  & 1.57 \\ \hline
    \multirow{3}[6]{*}{CIFAR10} & FNNSmall & 0.69  & 0.48  & 0.41  & 0.40  & 0.38  & 0.35  & 0.33  & 0.26  & 0.25  & 0.22 \\ \cline{2-12}          
                                & FNNMed & 1.13  & 0.65  & 0.73  & 0.43  & 0.40  & 0.30  & 0.63  & 0.27  & 0.18  & 0.24 \\\cline{2-12}          
                                & FNNBig & 2.08  & 1.03  & 0.62  & 0.65  & 0.65  & 0.27  & 0.25  & 0.24  & 0.11  & 0.13 \\
    \hline
    \end{tabular}%
  \label{tab:avgcosts}%
\end{table*}%

\noindent \emph{RQ4: How does the value of $\eta$ influence the repair results?} At line 8 of
Algorithm~\ref{alg:repair}, we `repair' a neuron by subtracting $\eta\cdot\nabla$ from its output $\zeta$. The parameter $\eta$ has
a great impact on the repair results in many ways. Intuitively, the larger $\eta$ is, the bigger the modification is, which may have consequences on the
fidelity or accuracy as well as the success rate of the repair. Deciding the optimal value for $\eta$ is
highly non-trivial. In the following, we apply \textsc{nRepair} with different $\eta$ to understand its impact and subsequently provide practical
guidelines on how to set the value of $\eta$. 

Concretely, for the ACAS Xu models, we evaluate the influence of $\eta$ on three representative models, one for each of the three properties, i.e., model $N_{3,8}$, $N_{1,9}$ and $
N_{2,9}$ for property 2, property 7 and property 8 respectively. Note that the model for property 2, i.e., $N_{3,8}$, is selected
according to the median of the number of partitions. For MNIST and CIFAR10, we take all the three models, i.e., FNNSmall, FNNMed and FNNBig, and for each target model, to evaluate
the effect of $\eta$. For each model, we set $\eta$ to 10 different values, i.e., from 0.05 to 0.5 with a step size of 0.05, and then evaluate the
effects from three aspects, i.e., success rate, fidelity/accR and time overhead. In the following, we show the results in the
three aspects separately.

\textit{Influence on success rate}. The results of the success rate are shown in
   Table~\ref{tab:sr}. It can be observed that the sensitivity to the value of
   $\eta$ varies across different repair cases. Concretely, for small models, e.g., FNNSmall of MNIST and CIFAR10, $\eta$ has limited impact and the success rate remains unchanged.
   %  Concretely, for some models of ACASXU and FNNSmall of MNIST, the success rate remains unchanged, i.e., 100\%.  
   For the middle-size models of MNIST and CIFAR10, the success rate
   fluctuates between 96\% and 100\% with the increasing of $\eta$. For the large models, the success rate drops
   gradually with the increasing of $\eta$, although not monotonically. %In the following, we will discuss the three sorts of results.

Our hypothesis is that for simple models, which can be repaired by modifying a small number of neurons, there is a threshold of $\eta$ such
that the magnitude of modification is adequate to ``repair'' the neuron. Let us imagine the model could be repaired if one neuron's output is below (or beyond) a threshold. 
In such a case, as long as $\eta$ is sufficiently large, the success rate remains unchanged. %Note that this hypothesis holds when the number of modified neurons is fewer. 
When multiple neurons are modified, it is possible that the modification on the neurons may influence each other (due to their correlations). This perhaps explains why in some cases, 
i.e., the middle-size models of MNIST and CIFAR10, the success rate fluctuates. For big
models, the declines of success rate is likely due to the fact that the number of modified neurons increase, and their correlations are complicated, as well as the overall search is 
big and complex and thus solving the optimization defined in Formula~\ref{fm:repair} is much more challenging. %In this case, a larger $\eta$ can make the algorithm overstep the local minima.
% \dgl{show the modifed neurones}  

\textit{Influence on the performance of repaired models}. We also explore the impact of $\eta$ on the ``generalizability'' of the repaired
  models, i.e., how big an impact on the global accuracy the repair would lead to with different $\eta$. The results are shown in Figure~\ref{fig:quality}. 
  As expected, the performance, i.e., fidelity or accR, decreases with
  the increasing of $\eta$ in general, although the magnitude of the decline differs from model to model. Concretely, for small models, e.g.,
  FNNSmall for both MNIST and CIFAR10, are insensitive to the value of $\eta$. That is, their performance decreases slightly
  (1.76\% decline for MNIST and 3.74\% decline for CIFAR10). For big models, the performance of repaired results
  drops significantly when the value of $\eta$ increases. This result is expected as a larger $\eta$ means a greater
  modification during each iteration in Algorithm~\ref{alg:repair}. Furthermore, as discussed above, deeper and larger networks tend to magnify small modification.  
  
 \textit{Influence on time overhead}. Intuitively, a larger $\eta$ may accelerate the repair. We show the average time
  of successfully repair in Table~\ref{tab:avgcosts}. We can observe that in most cases, the time overhead decreases
  when an increased $\eta$ value. Specially, for the FNNBig of CIFAR10, the time overhead decreases significantly, e.g., the repair with
  0.5 on FNNBig is 16 times faster than that with $0.05$. However, there is an exception where the costs increase, i.e., FNNMed of
  MNIST. This is because that the a large $\eta$ may lead to over modification on a single neuron and make the
  neuron ``jump over" the ``solution". In this case, more neurons will be involved, and thus more time are spent. We thus have the following answer to RQ4.
  
\begin{comment}
The experiment results are shown in Figure~\ref{fig:rq2} where the y-axis is the fidelity and (relative) accuracy of the repaired
model, which measures the impact of $\epsilon$. It can be observed that with the increasing of $\epsilon$, the performance, i.e.,
fidelity or (relative) accuracy,  of these models decreases in general, as expected. However, the rate of decreasing vary across
different models and the performance, is not monotonically decreasing. In some cases, the performance increases with a larger
$\epsilon$, e.g., the fidelity of $N_{5,1}$ increases when $\epsilon$ is increased from 0.3 to 0.5. One hypothesis is that this
could be due to the fact that the effect of the `activating' some of the neurons is canceled by `deactivating' the other neurons
(when line 7 in Algorithm~\ref{alg:optmize} is applied). We have the following answer to RQ3.
\end{comment}

\begin{framed}
\noindent \emph{Answer to RQ4: In general, a small $\eta$ leads to a repaired model with a high fidelity and more time spent on repairing. Our practical guideline is thus to 
have a small $\epsilon$ as long as the model can be repaired.}.
\end{framed}


%. We also observe that for in some subfigures, i.e.,  ``MNIST-FNNMed'', there exists a repair case the fidelity of which remains
%unchanged when varying the $\epsilon$. This is caused by the action of deactivation. Concretely, recall the
%Algorithm~\ref{alg:repair}, when the sign of a selected neurone is positive, we perform the deactivation on the neuron by setting
%its output as 0 at line 7, which is $\epsilon$-free. Thus, if a repair succeeds before the action of activating performed, then
%the repair is always independent from the value of $\epsilon$.



% Table generated by Excel2LaTeX from sheet 'time overhead' \begin{table}[htbp] \centering \caption{Add caption}
%\begin{tabular}{|c|l|r|r|r|} \hline \multirow{3}[6]{*}{ACASXU} & repair cases & 375   & 11    & 10 \\
%\cline{2-5}          & total(min) & 728   & 57    & 21 \\
%\cline{2-5}          & avg(min) & 1.94& 5.18 & 2.1 \\
%    \hline \multirow{3}[6]{*}{MNIST} & repair cases & 100   & 100   & 51 \\
%\cline{2-5}          & total(min) & 10    & 46    & 40 \\
%\cline{2-5}          & avg(min) & 0.1   & 0.46  & 0.78\\
%    \hline \multirow{3}[6]{*}{CIFAR10} & repair cases & 100   & 100   & 100 \\
%\cline{2-5}          & total(min) & 4     & 13    & 11 \\
%\cline{2-5}          & avg (min) & 0.04  & 0.13  & 0.11 \\
%    \hline \end{tabular}% \label{tab:addlabel}% \end{table}%


% Table generated by Excel2LaTeX from sheet 'modifed_neurones' \begin{table*}[t] \centering \caption{Number of modified neurones
%with different $\epsilon$} \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|} \hline Group & Model & Repair case & 0.5   & 1     & 1.5   &
%2     & 2.5   & 3     & 3.5   & 4 \\
%    \hline \multirow{12}[24]{*}{group1} & \multirow{4}[8]{*}{n28} & r1 & 1     & 1     & 3     & 3     & 3     & 3     & 4  & 3
%    \\ \cline{3-11} &       & r2 & 3     & 3     & 2     & 2     & 2     & 8     & 8     & 8 \\
%\cline{3-11}          &       & r3 & 1     & 1     & 6     & 6     & 6     & Failed & 9     & 9 \\
%\cline{3-11}          &       & r4 & 2     & 2     & 5     & 5     & 5     & 6     & 6     & 6 \\
%\cline{2-11}          & \multirow{4}[8]{*}{n49} & rc1 & 3     & 1     & 2     & 6     & 2     & 6     & 6     & 6 \\
%\cline{3-11}          &       & r2 & 1     & 1     & 1     & 1     & 4     & 4     & 2     & 4 \\
%\cline{3-11}          &       & r3 & 1     & 1     & 1     & 1     & 1     & 1     & 1     & 1 \\
%\cline{3-11}          &       & r4 & 1     & 1     & 1     & 1     & 5     & 5     & 6     & 7 \\
%\cline{2-11}          & \multirow{4}[8]{*}{n58} & rc1 & 4     & 1     & 1     & 1     & 1     & 1     & 1     & 1 \\
%\cline{3-11}          &       & r2 & 2     & 1     & 1     & 1     & 1     & 1     & 1     & 1 \\
%\cline{3-11}          &       & r3 & 2     & 2     & 2     & 2     & 2     & 2     & 2     & 2 \\
%\cline{3-11}          &       & r4 & 1     & 1     & 1     & 1     & 1     & 2     & 2     & Failed \\
%    \hline \multirow{3}[6]{*}{group2} & n22   & rc1   & 5     & 1     & 1     & 1     & 1     & 1     & 1     & 1 \\
%\cline{2-11}          & n43   & rc1   & 3     & 4     & 4     & 8     & 8     & 10    & 3     & 3 \\
%\cline{2-11}          & n47   & rc1   & 5     & Failed & 9     & 9     & Failed & 9     & 9     & 4 \\
%    \hline \end{tabular}% \label{tab:rq2-mn}% \end{table*}%

%\begin{figure}[t] \begin{subfigure}{\textwidth} %             \centering
%     \includegraphics[width=0.25\textwidth]{figs/rq2/acas-n28.pdf} \includegraphics[width=0.25\textwidth]{figs/rq2/acas-n49.pdf}
%     \end{subfigure} \begin{subfigure}{\textwidth} %             \centering
%     \includegraphics[width=0.24\textwidth]{figs/rq2/acas-n58.pdf}
%     \includegraphics[width=0.24\textwidth]{figs/rq2/acas-group2.pdf} \end{subfigure} \caption{The fidelity of repaired models
%     with different $\epsilon$} \label{fig:rq2-fdlt} \end{figure}


% \noindent \emph{RQ5: How to choose the value of $\alpha$ and $\beta$?} To recap, $\alpha$ denotes the maximum number of neurons
% allowed to modify and $\beta$ controls how many times a neuron can be modified. 
% The two parameters together 


\subsection{Threats to Validity}
\noindent \emph{The dependence on the verifier} We only evaluate our approach with the DeepPoly verifier. We choose DeepPoly as
it is the state-of-the-art at the time of writing. Different verifiers may lead to different performance. In fact, our approach is
orthogonal to the rapid development of neural network verification techniques. As long as the verifier used in our framework is
sound (i.e., when the verifier returns holds, the property actually holds), our approach works. \\ 

\noindent \emph{The size of repaired network} As illustrated in Algorithm~\ref{alg:overall},  our approach returns an
repaired network which is the result of assembling the repaired result of each erroneous partition. Thus, the size of the final repaired network depends on
the number of erroneous partitions. In our experiments, for the ACAS Xu DNNs, the number of partitions
varies from 2 to 20, and thus the size of the repaired network is 2 times to 20 times bigger than the original one. The blowup
could be reduced by combining common parts of the repaired network, which we will study in the future work. \\

\noindent \emph{Limited number of images} We evaluate our approach with 100 images in fixing the local robustness property. The
amount of images may not be adequate. Our experimental setting is largely adopted from existing work, i.e., Goldberger \emph{et al.}~\cite{mm} and
Singh \emph{et al.}~\cite{deeppoly}, both used 100 images for evaluation. In our experiments, we take the limited number of images because that
it is difficult to obtain qualified test cases. Images selected from the testing dataset must be correctly predicted by the
original model but fail to be verified. Meanwhile, at least one counterexample can be found when one image can not be verified.
Under these constraints, the total number of qualified images is small. For example, we only found 51 qualified
images for the FNNBig on the whole MNIST testing set (10000 images in total). However, our approach can be easily extended
to large scale datasets if more qualified images are available.

  
% % the authors lack comparison on multiple types of perturbations. For instance, how does the model perform on spatial, \ell_2 and
% % \ell_1 attacks?

% it is hard to validate the outstandingness of the proposed model due to the lack of comparison with relevant baselines for
% verification of networks. The authors highlight the relevant works including [Goldberger et al., Singh et al.], however, they do
% not provide any empirical comparisons with these to highlight the contributions of their work

% Why only 100 images were used for repair? Did the authors try to increase the attack strength and evaluate the repair technique for a large set of images?

% We agree with the reviewer that more images and stronger attacks will strengthen the evaluation. The current experimental setting
% is largely adopted from existing work, i.e.,., Goldberger et al., Singh et al, both of which used 100 images for evaluation. We
% are currently evaluating our approach against PGD attack.

